Analyzing Fundamental Diagrams of Mixed Traffic Control at Unsignalized Intersections

This report examines the effect of mixed traffic, specifically the variation in robot vehicle (RV) penetration rates, on the fundamental diagrams at unsignalized intersections. Through a series of simulations across four distinct intersections, the relationship between traffic flow characteristics were analyzed. The RV penetration rates were varied from 0% to 100% in increments of 25%. The study reveals that while the presence of RVs influences traffic dynamics, the impact on flow and speed is not uniform across different levels of RV penetration. The fundamental diagrams indicate that intersections may experience an increase in capacity with varying levels of RVs, but this trend does not consistently hold as RV penetration approaches 100%. The variability observed across intersections suggests that local factors possibly influence the traffic flow characteristics. These findings highlight the complexity of integrating RVs into the existing traffic system and underscore the need for intersection-specific traffic management strategies to accommodate the transition towards increased RV presence.

==> sections/experiment.tex <==
\section{Experimental Setup}
\label{sec:exp}

To evaluate the proposed model, we follow the same data processing procedures as the STA-LSTM model. Each vehicle trajectory is downsampled by a factor of 2, and the coordinate space centered around the target vehicle is discretized into a $3 \times 13$ spatial grid, where the $y$-axis represents the highway's motion direction and $x$-axis represents the highway lane encoding. A time step of 0.2 seconds is used.

For data preparation, we considered 15-step (3-second) historical trajectories of the target and neighboring vehicles within the $3 \times 13$ grid as inputs. The task is to predict the next 5-step (1-second) future trajectory of the target vehicle. This process minimizes the following objective:

\begin{equation}
L(\theta) = \frac{1}{N} \sum_{i=1}^{N} \sum_{t=1}^{T} \left[ (\hat{x}_{i,t} - x_{i,t})^2 + (\hat{y}_{i,t} - y_{i,t})^2 \right] \\
\end{equation}
\renewcommand{\labelitemi}{}
\begin{itemize}
    \item $N$ = Number of training samples
    \item $T$ = Number of predicted time steps
    \item $(\hat{x}_{i,t}, \hat{y}_{i,t})$ = Predicted coordinates for sample $i$ at time step $t$
    \item $(x_{i,t}, y_{i,t})$ = Actual coordinates for sample $i$ at time step $t$
    \item $L(\theta)$ = MSE on Euclidean distance
\end{itemize}
\vspace{1cm}
For model configuration, the embedding size is set to 32, while the LSTM hidden state dimension is set to 64. The feed-forward layer in the Transformer encoder has a dimension of 512. We train the model using the Adam optimizer with a learning rate of 0.001. The model is trained for 50 epochs on an Intel i9-14900K CPU, an Nvidia GTX 4090 GPU, and 32GB RAM. The total training time is approximately 15 hours. These settings ensure a fair comparison with the STA-LSTM model while leveraging the extended feature representation provided by the Transformer-enhanced architecture.

==> sections/related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Traditional Methods for Trajectory Prediction}
Conventional approaches to vehicle trajectory prediction include physics based, maneuver based, and interaction-aware models. Physics based methods rely on kinematic and dynamic constraints such as acceleration, yaw rate, and road friction to predict short-term trajectories. While accurate for minimal time horizons, these models often fail to account for complex driver behaviors or interactions with surrounding vehicles \cite{c8}. Maneuver based models enhance physics based methods by incorporating predefined driver intentions, such as lane changes or turns, to improve prediction accuracy as in \cite{c9}. However, both approaches are limited in capturing interactions among vehicles, a critical factor in crowded or dynamic traffic environments.

\subsection{Deep Learning Approaches with LSTMs}
The advent of deep learning has revolutionized trajectory prediction by enabling data-driven modeling of complex temporal and spatial dependencies. Long Short-Term Memory (LSTM) networks, a class of recurrent neural networks, have been widely adopted due to their ability to model long-term dependencies in sequential data.

For example, Deo and Trivedi \cite{c4} proposed a convolutional social pooling LSTM model that considers vehicle interactions for trajectory prediction by aggregating spatial features from surrounding vehicles. This approach demonstrated the potential of LSTMs in managing traffic dynamics through multi-agent interactions.

To enhance context-awareness, STA-LSTM integrates spatiotemporal attention mechanisms, allowing the model to assign attention weights to both historical trajectories and neighboring vehicles. This enhances interpretability and provides valuable insights into the factors influencing the target vehicle’s future motion. The spatial attention mechanism focuses on nearby vehicles, while temporal attention tracks the influence of past trajectory points.

Further advancements in LSTM based trajectory models include the Social GAN proposed by Gupta et al. \cite{c13}, which models human-like interactions using LSTM based encoders and decoders combined with generative adversarial networks. Similarly, Sadeghian et al. \cite{c14} introduced Sophie, a socially-aware trajectory prediction framework that leverages LSTMs with attention mechanisms and semantic scene contexts for better prediction in complex environments.

More recently, Amirian et al. \cite{c15} extended LSTM based methods by integrating variational autoencoders (VAEs) to model trajectory uncertainty, demonstrating the flexibility of LSTMs in probabilistic forecasting. Such models enable dynamic uncertainty estimation in real-world scenarios where trajectory outcomes are inherently uncertain due to unpredictable human behavior.

These works underscore the continued relevance and adaptability of LSTM based models in trajectory prediction, especially when integrated with attention mechanisms, social pooling, and probabilistic components.

\subsection{Transformer Models for Trajectory Prediction}
Transformer models have emerged as a groundbreaking approach in time-series modeling due to their ability to capture long-range dependencies through self-attention mechanisms \cite{c6}. Unlike LSTMs, which process sequences sequentially, Transformers evaluate all elements of a sequence simultaneously, enabling efficient modeling of complex vehicle interactions in traffic environments. This characteristic makes Transformers well-suited for tasks involving simultaneous spatial and temporal reasoning.

The self-attention mechanism in Transformers dynamically assigns importance weights across the entire sequence, allowing the model to focus on key features at different time steps. This capability makes Transformers advantageous for modeling complex vehicle-vehicle and vehicle-environment interactions, where dependencies can occur across non-adjacent time steps \cite{c8}.

Zhou et al. \cite{c7} demonstrated the potential of Transformers in long-sequence time-series forecasting, highlighting their ability to integrate both global and local feature patterns. Their work emphasized how self-attention enables the effective aggregation of contextual information across extended prediction horizons. Similarly, Liu et al. \cite{c11} showed that Transformers outperform traditional RNNs in capturing intricate temporal relationships in dynamic systems.

In trajectory prediction, where interaction-aware modeling is crucial, applying Transformer architectures can provide a robust framework for predicting multi-agent trajectories. Recent work by Chen et al. \cite{c12} illustrated how attention based architectures improved trajectory forecasting by learning high-level spatiotemporal interactions, paving the way for more interpretable and accurate autonomous driving models.
